Gaussian Splatting in Mirrors: Reflection-Aware Rendering via Virtual Camera Optimization

Recent advancements in 3D Gaussian Splatting (3D-GS) have revolutionized novel view synthesis, facilitating real-time, high-quality image rendering. However, in scenarios involving reflective surfaces, particularly mirrors, 3D-GS often misinterprets reflections as virtual spaces, resulting in blurred and inconsistent multi-view rendering within mirrors. Our paper presents a novel method aimed at obtaining high-quality multi-view consistent reflection rendering by modelling reflections as physically-based virtual cameras. We estimate mirror planes with depth and normal estimates from 3D-GS and define virtual cameras that are placed symmetrically about the mirror plane. These virtual cameras are then used to explain mirror reflections in the scene. To address imperfections in mirror plane estimates, we propose a straightforward yet effective virtual camera optimization method to enhance reflection quality. We collect a new mirror dataset including three real-world scenarios for more diverse evaluation. Experimental validation on both Mirror-Nerf and our real-world dataset demonstrate the efficacy of our approach. We achieve comparable or superior results while significantly reducing training time compared to previous state-of-the-art.

==> cmzwcrkpgcphjynvzfzymcqsmrtmhycx/sec/exps.tex <==
\section{Experiments}

\subsection{Training Details}

Most of the experiments conducted in this paper are on a single V100 GPU and using the pytorch framework (Only the rendering speed (FPS) is tested on a single RTX 4090 GPU), with a total of 60,000 training steps. For all the experiments, the regularization weights are set as follows: $\lambda_{s} = 0.01$, $\lambda_{n} = 0.005$, $\lambda_{pc} = 0.01$, and $\gamma = 0.1$. We employed the Adam Optimizer~\cite{kingma2014adam} for virtual camera optimization, setting the learning rate at 0.0005. The total number of steps for the mirror plane prediction stage was 1000 for experiments conducted on Mirror-NeRF's synthetic dataset and our dataset, and 1500 for Mirror-NeRF's real dataset. The virtual camera optimization stage consisted of 10,000 steps. Please refer to the supplementary for the implementation details.

\subsection{Experimental Results}

\noindent
\textbf{Dataset.} We evaluate our method using the publicly available Mirror-Nerf dataset~\cite{zeng2023mirror}, which includes three synthetic scenes (Washroom, Living room, Office) and three real scenes (Market, Lounge, Discussion room). Each scene is captured within a room containing mirror, with approximately 300 frames taken from a 360-degree perspective. The dataset also includes a mirror reflection mask in each image. 
To enhance the evaluation of our method in real-world scenarios, we provide an additional dataset containing three scenes, Recovery Room, Work Space, and Corridor, with the mirror size and shape in each scene being different from others. The dataset comprises 250 frames per scene, with mirror reflection masks extracted using SAM~\cite{kirillov2023segment} and camera poses estimated by COLMAP~\cite{schonberger2016structure}. We follow ~\cite{zeng2023mirror} to split the training and test dataset and each set includes a mix of views with and without mirror. We show the example images of the mirror scenes from simple to complex in the supplementary.

\noindent
\textbf{Baselines and Evaluation Protocol.} We consider the following methods as baselines for comparison (a) start-of-the-art Mirror-NeRF~\cite{zeng2023mirror}; two fast-rendering methods (b) InstantNGP~\cite{muller2022instant} and  (c) DVGO~\cite{sun2022direct} and (d) the official 3DGS~\cite{kerbl20233d}. Following the standard practice in novel view synthesis, we evaluate the rendering quality using the metrics PSNR, SSIM~\cite{wang2004image} and LPIPS~\cite{zhang2018unreasonable}.

\subsubsection{Mirror-NeRF Dataset Results}
Table.~\ref{tab:mirror-nerf} presents the experimental results for Mirror-Nerf~\cite{zeng2023mirror} synthetic and real datasets. On the synthetic dataset, our method outperforms the best method, Mirror-NeRF, in both PSNR and SSIM metrics, achieving state-of-the-art performance. This success is largely due to our mirror plane prediction described in Section \ref{sec:Mirror Plane Prediction}, which effectively initializes the plane equation on synthetic datasets. The subsequent virtual camera optimization further enhances the rendering quality. Compared to the vanilla 3D-GS, our method achieves significant improvement with the average values across three scenes. Specifically, in the office scene, our method shows gains of +8.65 in PSNR, +0.057 in SSIM, and -0.067 in LPIPS.

On real datasets,  our method approaches the performance of Mirror-NeRF, with significantly faster rendering speed (FPS 128.22 v.s. 0.71). Compared to more efficient rendering methods like InstantNGP~\cite{muller2022instant} and DVGO~\cite{sun2022direct}, the proposed approach leads in all metrics with a large margin, indicating that our method can provide both high-quality and efficient image rendering. We provide the qualitative comparison in Fig.~\ref{fig:vis.pdf}, and our method achieves high rendering quality with less blurred regions. 

\subsubsection{Our Real-World Dataset Results}

Table.~\ref{tab:custom} presents the comparative results of vanilla 3D-GS and our method on the proposed dataset. In the Corridor and Recovery Room scene which contains large mirrors and planer surface, our method significantly outperforms 3D-GS on all the metrics. 3D-GS estimates mirror reflections as virtual spaces behind the mirror plane, necessitating extensive optimization of additional Gaussians within this virtual space. This results in blurry details and textures, since the resulting mirror regions are not multi-view consistent. Conversely, our method does not require the optimization of additional Gaussians to explain mirror reflections and facilitates more physically accurate mirror rendering using virtual cameras resulting in better detail preservation in the scene.

However, in the Work Space scene, our method exhibits a slight decline relative to 3D-GS. This scene is characterized by a large, cluttered space filled with numerous items, which poses challenges for our method due to the absence of planer surfaces for depth or normal supervision. Consequently, it struggles to derive an effective mirror equation, leading to discrepancies in the virtual camera pose estimation and less effective virtual camera rendering compared to 3D-GS. This highlights areas where further refinement of our method is needed to handle complex scenarios effectively.

\begin{table*}[t!]
\small
\renewcommand\arraystretch{1.3}
\begin{center}
\resizebox{.85\textwidth}{!}
{
\begin{tabular}{lcccclccc}
\toprule 
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Synthetic}}             &  & \multicolumn{3}{c}{\textbf{Real}}                 \\
                         & PSNR  $\uparrow$         & SSIM  $\uparrow$         & LPIPS  $\downarrow$        & FPS $\uparrow$ &  & PSNR  $\uparrow$         & SSIM  $\uparrow$         & LPIPS  $\downarrow$           \\ \midrule
InstantNGP~\cite{muller2022instant}               & 23.54          & 0.71           & 0.42           & - &  & 10.51          & 0.20           & 0.71           \\
DVGO~\cite{sun2022direct}                     & 28.05          & 0.82           & 0.29           & - &  & 22.18          & 0.67           & 0.33           \\
Mirror-NeRF~\cite{zeng2023mirror}               & \underline{38.08}    & \underline{0.958}    & \textbf{0.028} & 0.71 &  & \textbf{25.31} & \textbf{0.789} & \textbf{0.082} \\ \midrule
3D-GS~\cite{kerbl20233d}                     & 36.52          & 0.953          & 0.064          & \textbf{480.29} &  & 23.39          & 0.715          & 0.268          \\
\textbf{Ours}            & \textbf{39.87} & \textbf{0.979} & \underline{0.038}    & \underline{128.22} &  & \underline{24.19}    & \underline{0.759}    & \underline{0.234}    \\ \bottomrule

\end{tabular}
}
\end{center}
\caption{Results on the Mirror-NeRF's synthetic and real-world dataset, our method approaches or achieves state-of-the-art performance on these two datasets, and significantly improves upon 3D-GS. The FPS values are measured on an RTX 4090 GPU. The best result is in \textbf{bold}, and the second best is \underline{underlined}.}
\label{tab:mirror-nerf}
\end{table*}

\begin{table}[t!]
\renewcommand\arraystretch{1.3}
\begin{center}
\resizebox{.9\textwidth}{!}
{
\begin{tabular}{lccclccclccc}
\toprule
\multirow{2}{*}{\textbf{Method}}             & \multicolumn{3}{c}{\textbf{Corridor} (easy)}                      &  & \multicolumn{3}{c}{\textbf{Recovery Room} (medium)}        &  & \multicolumn{3}{c}{\textbf{Work Space} (complex)}                           \\
                                     & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ &  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ &  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ \midrule
3D-GS~\cite{kerbl20233d} & 25.9           & 0.845           & 0.332              &  & 28.84           & 0.917           & 0.166     &  & \textbf{26.88}  & \textbf{0.884}  & \textbf{0.219}             \\
Ours                                 & \textbf{29.14}  & \textbf{0.874}  & \textbf{0.291}     &  & \textbf{32.21}  & \textbf{0.938}  & \textbf{0.139}              &  & 24.89           & 0.849           & 0.288    \\ \bottomrule

\end{tabular}
}
\end{center}
\caption{Results on the our real-world mirror dataset. Our proposed method outperforms vanilla 3D-GS on two of the scenes. The best result is marked with \textbf{bold}.}
\label{tab:custom}
\end{table}

\begin{figure*}[t!]
\begin{center}
\includegraphics[width=1.0\linewidth]{vis.pdf}
\vspace{-1em}
\end{center}
   \caption{Qualitative comparisons of ground truth, 3D-GS, and our method on the Living Room, Office, Lounge, Corridor, and Recovery Room scenes from Mirror-NeRF dataset. The smaller image in the upper right corner of each main images is an enlargement of a mirror region.}
\label{fig:vis.pdf}
\end{figure*}

\subsection{Ablation Study}
We present the ablation study on loss function selection and virtual camera optimization strategies in Table.~\ref{ablation}. The experiments demonstrate that removing any loss function related to the depth map or normal map in plane prediction significantly reduces the accuracy of rendering quality. Removing the normal loss shows the worst performance, indicating the effectiveness of the proposed depth and normal optimization. Additionally, without virtual camera optimization leads to a notable decline in rendering quality. This underscores the critical role of camera optimization in refining both the mirror plane and the virtual camera pose, especially when the initial plane prediction is imperfect. Furthermore, we conduct ablation study on the joint virtual camera and Gaussians optimization. The results demonstrate that this joint optimization detracts from the rendering quality, confirming our assumptions discussed in Sec.~\ref{sec:Virtual Camera Optimization}. 

% In mirror plane estimation, we randomly select a view with a large mirror region and then use this view to estimate the mirror plane. To further investigate whether this random selection affects the quantitative results, we conduct an additional ablation study. Specifically, we utilize the \textit{Living Room} scene from the Mirror-NeRF dataset and randomly choose 5 different views for plane estimation. Each view is trained using the same settings as outlined in our paper, and the metrics are computed as presented in Table~\ref{tab:random}. The results suggest that varying the selected views has minimal impact on the final rendering quality, underscoring the robustness of our approach in accommodating random view selection scenarios.



\begin{table}[t!]
\renewcommand\arraystretch{1.1}
\begin{center}
\resizebox{.6\textwidth}{!}
{
\begin{tabular}{c|ccc}
\toprule
\textbf{Settings}                        & \textbf{PSNR} $\uparrow$          & \textbf{SSIM} $\uparrow$          & \textbf{LPIPS} $\downarrow$         \\ \midrule
w/o $\mathcal{L}_{n}$                     & 32.30          & 0.964          & 0.071          \\
w/o $\mathcal{L}_{pc}$                      & 32.51          & 0.956          & 0.069          \\
w/o $\mathcal{L}_{smooth}$                   & 34.49          & 0.967          & \textbf{0.037} \\
w/o Camera Optimization & 30.79          & 0.943          & 0.102          \\
Camera + Gaussians Optimization & 31.30          & 0.940         & 0.103          \\
Full  Model                     & \textbf{37.30} & \textbf{0.977} & 0.042          \\ 
\bottomrule
\end{tabular}
}
\end{center}
\caption{Ablation studies of various components of our proposed approach using the Office scene form Mirror-NeRF dataset. The highest score is in \textbf{bold}.}
\label{ablation}
\vspace{-10pt}
\end{table}

% \begin{table}[]
% \begin{center}
% \begin{tabular}{cccc}
% \toprule
% \textbf{Scene} & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\ \midrule
% Living\_room   & 43.57 ± 0.321   & 0.992 ± \(6.9 \times 10^{-7}\)   & 0.011 ± \(4 \times 6^{-6}\)    \\ \bottomrule
% \end{tabular}
% \end{center}
% \caption{Ablation study result for different view selection in mirror plane estimation.}
% \label{tab:random}
% \end{table}
